Spend Your Rollouts Where It Counts: Rollout Allocation for Group-Based RL Post-Training

Reinforcement learning (RL) is the dominant paradigm for post-training large language models. However, in the online, on-policy setting, rollout generation dominates the computational cost of training. Group-based policy optimization methods compute advantages from multiple rollouts per prompt, yet they indiscriminately allocate budget to prompts with collapsed reward distributions, wasting expensive rollouts on negligible learning signals. We demonstrate that group-based updates are most effective in regimes of high reward variance. Since the policy evolves throughout training, prompt informativeness must be estimated online rather than precomputed, but exhaustively evaluating every prompt is computationally prohibitive. We introduce Pilot-Commit, a budget-aware rollout allocation framework for group-based RL post-training. Pilot-Commit decouples prompt evaluation from exploitation: a pilot stage estimates per-prompt informativeness using a fraction of the budget, and the remaining rollouts are allocated to high-leverage prompts while low-signal prompts are skipped. Across multiple math reasoning benchmarks and model scales from 1.5B to 14B parameters, Pilot-Commit matches baseline accuracy with significantly lower sampling costs, reaching target accuracy up to $1.9\times$ faster than GRPO and $4.0\times$ faster than DAPO in cumulative rollouts.

==> Makefile <==
all:
	@if command -v latexmk >/dev/null 2>&1; then \
		latexmk -pdf -interaction=nonstopmode main.tex; \
	elif command -v pdflatex >/dev/null 2>&1 && command -v bibtex >/dev/null 2>&1; then \
		pdflatex -interaction=nonstopmode main.tex && \
		bibtex main && \
		pdflatex -interaction=nonstopmode main.tex && \
		pdflatex -interaction=nonstopmode main.tex; \
	else \
		echo "Error: no TeX toolchain found. Install latexmk or pdflatex+bibtex."; \
		exit 1; \
	fi

clean:
	@if command -v latexmk >/dev/null 2>&1; then \
		latexmk -C; \
	else \
		rm -f main.aux main.bbl main.blg main.fdb_latexmk main.fls main.log main.out main.pdf; \
	fi

